URIE: Universal Image Enhancement for Visual Recognition in the Wild

Despite the great advances in visual recognition, it has been witnessed that recognition models trained on clean images of common datasets are not robust against distorted images in the real world. To tackle this issue, we present a Universal and Recognition-friendly Image Enhancement network, dubbed URIE, which is attached in front of existing recognition models and enhances distorted input to improve their performance without retraining them. URIE is universal in that it aims to handle various factors of image degradation and to be incorporated with any arbitrary recognition models. Also, it is recognition-friendly since it is optimized to improve the robustness of following recognition models, instead of perceptual quality of output image. Our experiments demonstrate that URIE can handle various and latent image distortions and improve the performance of existing models for five diverse recognition tasks when input images are degraded.

==> _1_introduction_backup_20200303.tex <==
% !TEX root = TY_ECCV20.tex
\section{Introduction}\label{sec:intro}

% \suha{this section is in progress and will be revised later; any comments are welcome. also add references.}

% \suha{image restoration vs. image enhancement}

% ======================================================================
% \recap{an issue of the recent approaches in visual recognition}
% + we have seen great advances in visual recognition thanks to the development of deep neural networks, but still have far way to go to achieve visual recognition in the wild
% + researchers have put efforts into improving performance in high quality images taken in limited environments, but in real world scenarios, visual data are often degraded by many factors including
%    - weather conditions (e.g., fog and rain)
%    - over- and under-exposure
%    - sensor noise
%    - motion blur
%    - compression artifcats
% + these are not considered when designing and training most of current SOTA models, thus they could be sensitive to such degradations
%    - it has been reported in literature that SOTA architectures are sensitive to image degradation (i.e., performance degraded when input image degraded)
%    - find and cite relevant papers other than ImnageNet-C paper
% + indeed we have to consider image quality degradation in testing time to build more realistic visual recognition models
% ======================================================================
The development of deep learning has made the great advances in visual recognition. 
% However, we still have a far way to go to achieve robust visual recognition in the wild. 
Especially, the recent advances in this field have been concentrated on accurate and comprehensive understanding of high-quality images taken in limited environments.
% However, most of the effort has been devoted to improve recognition performance on high-quality images taken in limited environments, 
However, images in the real world are often corrupted by various factors including adverse weather conditions, sensor noise, under- or over-exposure, motion blur, and compression artifact.
Since most of existing recognition models do not consider these factors, their performance could be easily degraded when input image is corrupted~\cite{dirtypixel,Hendrycks2019_ImageNetC,Zendel_2018_ECCV}, which could be fatal in safety-critical applications like autonomous driving. 

% The development of deep learning has made the great advances in visual recognition. \suha{references?}
% Especially, most of the advances have been concentrated on accurate and comprehensive understanding of high-quality images taken in limited environments.
% % However, most of the effort has been devoted to improve recognition performance on high-quality images taken in limited environments, 
% However, images in the real world are often corrupted by various factors like weather conditions (\eg, fog and rain), under- and over-exposure, sensor noise, motion blur, and compression artifact.
% Since most of state-of-the-art recognition models do not consider those factors, their performance would be degraded when input image is corrupted. \suha{cite ImageNet-C and any other relevant papers}
% Indeed, we still have a far way to go to achieve robust visual recognition in the wild. 
% % as a step towards xxx, we ...



% ======================================================================
% \recap{existing methods resolving this issue and their limitations}
% + image enhancement
%    - a straightforward way to resolve the above issue is to apply image enhancement models to input images before feeding them to the recognition models
%    - limitations
%       -- most existing methods handle a single type of image degradation (e.g., denoising, dehazing, deblurring, super-resolution); a few methods assume multiple and latent degradation types, but their performance is not satisfactory yet (find and cite relevant papers)
%       -- they are not optimized for visual recognition models; they are designed and trained to improve image quality by minimizing reconstruction errors, which do not guarantee the improvement of recognition accuracy of the model take the enhanced images (show image examples: better in terms of PSNR/RMSE, but worse in recognition accuracy, reconstruction of background is not useful)
% + low quality image recognition
%    - e.g., low resolution image recognition (CVPR'XX, ICCV'19)
%    - limitations
%       -- usually focuss on a single degradation type and a single recognition task
%       -- thus hard to be generalized to a large variation of potential image degradations in real world, and a variety of visual recognition tasks
% + image enhancement for visual recognition
%    - ???
% ======================================================================

A na\"ive way to resolve this issue would be to improve the quality of input image fed to recognition models through image restoration.
However, existing models for image restoration are in general not suited to this role for the following reasons.
First, most of restoration methods assume that images are degraded by a single and known factor of corruption (\eg, denoising, deblurring, dehazing, deraining, and super-resolution). 
It is thus not straightforward for them to handle realistic recognition scenarios where images can be corrupted by various factors whose types and intensities are latent. 
Second, they are not trained for visual recognition but for human perception.
Hence input images restored by them do not always guarantee performance improvement of recognition models as demonstrated in~\cite{dirtypixel,Li_2019_CVPR,Pei_2018_ECCV,vidal2018ug2}.
 % and shown in Fig.~\ref{fig:motiv}. 
Finally, most of image restoration networks are computationally heavy as they have no pooling operation, thus will make the entire system overly expensive.


% ======================================================================
% FIGURE START
% \begin{figure*} [!t]
% \centering
% % \includegraphics[width = 1 \textwidth]{figures/fig1.pdf}
% \fbox{\rule{0pt}{1.2in} \rule{1\linewidth}{0pt}}
% \caption{
% \suha{compare image enhancement and restoration qualitatively; restoration could be better in terms of PSNR/RMSE but worse in terms of recognition accuracy (\eg, reconstruction of background is not useful for improving recognition accuracy.}
% } 
% \vspace{-2mm}
% \label{fig:motiv}
% \end{figure*}
% FIGURE END
% ======================================================================


% ======================================================================
% \recap{the main goal and key ideas of this work}
% + we propose an image enhancement model dedicated to visual recognition models working in the wild
% + plug and play: once trained, applicable to any existing visual recognition models of different architectures and for different tasks (image classification, object detection, semantic segmentation) --> this is nothing but the universality mentioned below.
% + design principles
%    - recognition-aware: the goal of our model is to enhance the image quality for improving visual recognition accuracy, not for human perception
%    - handling multiple and latent degradations: in real world applications, it is unknown in advance which kinds of image degradation will happen in testing
%    - universally applicable: likewise, a single enhancement model must be universally applicable to different architectures of visual recognition models and to different recognition tasks so that one can plug and play our model to any existing pretrained networks for any visual recognition tasks; otherwise, we have to prepare enhancement models for every individual architectures and recognition tasks, which is infeasible.
%    - efficient (light-weight): since every input to visual recognition models will be pre-processed by such a model, the model must be light-weight and fast enough; otherwise, the additional computation burden given by the model will be significant.
% ======================================================================

This paper addresses the problem through a novel image enhancement model dedicated to robust visual recognition in the wild. 
Specifically, we keep the following properties in our mind when developing the model.
(1)~\emph{Universally applicable}: 
Our model aims to be attached to any existing recognition models to improve their robustness in any arbitrary situations without retraining them. 
To this end, it has to deal with various factors of degradation whose types and intensities are latent, and be applicable to diverse recognition tasks and models. 
(2)~\emph{Recognition friendly}: 
Our model should be optimized for improving performance of following recognition models, instead of making images looking more plausible.
(3)~\emph{Computationally efficient}:
The complexity of our model has to be low enough to minimize the computational burden it additionally imposes.


% ======================================================================
% \recap{implementation of the ideas}

% + to achieve the goal, we study a new neural net architecture and its training strategy
% + the proposed network architecture (handling multiple and latent degradations, light-weight)
%    - smaller compared to most enhancement networks and recognition models
%    - using the selective kernel trick for handling various factors of image degradation efficiently and effectively within a single feed-forward architecture
%       -- a series of convolution layers as an image enhancement procedure
%       -- each convolution layer actually has two paths to handle the input in two different ways
%          --- incorporating different normalization schemes as well as convolution weights trained separately since different degradations have to be addressed in different manners
%          --- their results are combined in a channel-wise manner; attentions drawn for each channel indicates how much important a path is to handle the input for the channel
%       -- a concatenation of the two different paths of enhancement results in a large number of combinations, and the attention dynamically and automatically determines which combination will be proper to address the input.
% + recognition aware learning of the enhancement model (recognition friendly, handling multiple and latent degradations, universally applicable)
%    - training for imagenet-c classification
%       -- trained for improving image classification performance of an image classification network on imagenet images corrupted by multiple types and levels of image degradation (cite imagenet-c paper)
%       -- learning with image classifier for a large scale image recognition to train a general image enhancement function; imagenet pretrained networks are used as general image representation for arbitrary visual recognition tasks, we also argue that our training scheme using imagenet-c is also possible to learn task-invariant and dataset-invariant image enhancement function by a large-scale training (not convincing enough...)
%    - using a subset of degradation types as seen corruption and keep the others as unseen corruptions used only for validation (to show that our model can handle degradations unseen during training)
% ======================================================================


% ======================================================================
% FIGURE START
\begin{figure*} [!t]
\centering
% \includegraphics[width = 1 \textwidth]{figures/fig_arch.pdf}
\includegraphics[width = 1 \textwidth]{figures/fig_arch_sym.pdf}
% \includegraphics[width = 1 \textwidth]{figures/fig_selective_path.pdf}
% \fbox{\rule{0pt}{2in} \rule{1\linewidth}{0pt}}
\caption{
Overall architecture of URIE. The selective enhancement modules are indicated by gray rectangles. Details of these modules are illustrated in Fig.~\ref{fig:selective_path}.
} 
\vspace{-2mm}
\label{fig:overall_arch}
\end{figure*}
% FIGURE END
% ======================================================================

To realize these ideas, we propose a Universal and Recognition-friendly Image Enhancement network, dubbed URIE, that deals with various and latent distortions efficiently and effectively.
% , whose architecture is illustrated in Fig.~\ref{fig:overall_arch}.
%, together with its training strategy. 
As illustrated in Fig.~\ref{fig:overall_arch}, it formulates image enhancement as a series of convolution layers resembling U-Net~\cite{unet}.
% A special feature of URIE is that its all convolution layers, except the first and the last, have two internal paths with separate parameters and normalization operations.
% Regarding a path from input to output as an individual image enhancement process, this feature enables URIE to learn a large variety of enhancement functions since the number of such paths increases exponentially as its depth grows. 
A special feature of URIE is the \emph{selective enhancement module}, which has two internal enhancement paths with separate convolution parameters and normalization operations.
Convolution layers of URIE, except the first and the last, are all given in the form of this selective module.
Regarding an entire path from input to output as an individual enhancement procedure, this module enables URIE to learn a large variety of enhancement functions since the number of such paths increases exponentially as its depth grows. 
Moreover, to deal with latent degradation type of input image, these modules draw attentions on their paths dynamically so that paths appropriate to address the input will get larger attention weights and contribute more to the final result.
These attentions are drawn for individual local patches of input image to enhance different image regions differently.
% This attention mechanism is applied to each local patch of input image separately to enhance different image patches differently.


\iffalse % suha - 20200301
We first present a new \emph{light-weight} network architecture \emph{handling various and latent factors of degradation} effectively. 
% Different image corruptions have been addressed typically by different enhancement procedures, but it is impractical to employ multiple enhancement networks for individual degradation types. 
% Instead, 
As illustrated in Fig.~\ref{fig:overall_arch}, our network formulates image enhancement as a series of convolution layers, each of which has two separate paths.
This architecture increases the number of possible enhancement procedures (\ie, the number of paths from input to output) exponentially as the network depth grows,
% , with roughly twice the number of parameters.
and consequently allows to address various types of image degradation with a single network.
Note that the two paths of each convolution layer have different normalization operations, batch normalization~\cite{Batchnorm} and instance normalization~\cite{Instancenorm}, since different feature statistics are required to handle different corruptions. 
Moreover, to deal with latent degradation type of input, the network draws attentions on the paths dynamically so that paths appropriate to address the input will get larger attention weights and contribute more to the final result.
% the outputs of the two paths are aggregated by channel-wise weighted summation, where the weights are determined by channel-wise attention module. >> to much details?
% overall, similar with SKNet, but different in that blah blah ... >> move to related work
\fi

In addition, we propose a new training method that enables URIE to be recognition-friendly as well as universal.
For training, URIE is coupled to an image classification network pretrained on the original ImageNet dataset~\cite{Imagenet}.
It is then trained in an end-to-end manner to improve the performance of the classifier on distorted images.
As training data, we adopt ImageNet-C~\cite{Hendrycks2019_ImageNetC}, in which images of the original ImageNet are degraded by 19 classes of distortion; we use 15 among them for actual training and keep the other 4 as unseen corruptions for testing. 
This training strategy confers upon URIE the recognition-friendly property since the training objective is not the perceptual quality of output but the recognition performance of the coupled classifier. 
Furthermore, we expect that training URIE on the large-scale dataset with a variety of corruptions allows it to be invariant to the task and architecture of the following recognition model, like ImageNet pretrained networks that have been widely used as general representation for various purposes~\cite{deconvnet,Oquab2014,vggnet}.

% Also, as ImageNet classification networks have been widely used as general representation for various purposes~\cite{vggnet,Oquab2014,deconvnet}, we expect that our network trained on the large scale ImageNet dataset with a variety of corruptions will learn image enhancement invariant to the task and architecture of the following recognition model. \suha{the last one is not super strong, how should we revise this argument?}



% ======================================================================
% \recap{achievements}
% + handling multiple latent degradations, as designed so
% + light-weight / recognition-aware 
%    - cheaper in terms of both the number of parameters and FLOPs, but better than SOTA enhancement networks handling latent degradations (cite) in terms of recognition accuracy given enhanced images
% + universality
%    - apply our enhancement model to imagenet-c classification with different recognition models other than what we used to train the module
%    - apply our enhancement model to object detection and semantic segmentation: ours is working for different recognition tasks, and of course, different architectures for the different tasks
%    - demonstrate that although our model is trained for imagenet-c classificaiton with resnet-xx, it works also for architectures other than the resnet-xx for the same task, and also for different architectures developed for different recognition tasks as well.
% ======================================================================

The efficacy of URIE is evaluated on \suha{five? six?} different recognition tasks, in which recognition models are pretrained on clean images and tested with URIE on corrupted ones with no finetuning. 
Experimental results demonstrate that URIE improves recognition performance in the presence of image distortions including those unseen during training, and regardless of target tasks and recognition networks coupled with it. 
URIE is also compared with the state-of-the-art image restoration model~\cite{OWAN_CVPR19} in the same setting, and outperforms the model in terms of both recognition accuracy and computational efficiency.
In summary, the contribution of our work is four-fold: \suha{may be too strong?}
\begin{itemize}
    \item We introduce a new method towards robust visual recognition. Our method improves robustness of existing recognition models without retraining them through a single and universal image enhancement module. 
    \item We propose a novel neural network architecture that can handle various and latent types of image distortions effectively and efficiently.
    \item We present a new training strategy that enables our enhancement model to be universally applicable and recognition-friendly.
    \item In our experiments, our model improves recognition performance of existing models substantially in the presence of various image distortions regardless of tasks and models it is tested on. 
\end{itemize}


%
% ======================================================================
% \recap{contributions and organization of this paper}
% ======================================================================
% Our paper is organized as follows. 
% Section~\ref{sec:relatedwork} reviews previous work motivating or closely related to ours.
% and Section~\ref{sec:method} describes the architecture of URIE and its training strategy in details.





==> _3_method_backup_20200302.tex <==
% !TEX root = TY_ECCV20.tex
\section{Our Framework} \label{sec:method}

% Method - Model Architecture(Our Framework)
%   - Using Instance norm and Batch norm 
%   - Selective Attention mechanism from SKNet
%   - ...
%
% Flow 
% - section 3. Our Model (model architecture 뭘로 갈거냐에따라 제목 바뀔 것)
% - brief overview
% - what are special in our model
% section 3.1. Model Architecture
% - overall architecture (convs / unet 아직 결정 안되었으니 두 버전으로 작성)
% - architecture details
% - mathematical expression of the network
% section 3.2. Training Scheme
% section 3.3. Discussion
% - how/why it works
% - comparison to SKNet
% - comparison to RL-Restore / OWAN


% We first present a newlight-weightnetwork architecturehandling various andlatent factors of degradation effectively. As illustrated in Fig. 2, our network for-mulates image enhancement as a series of convolution layers, each of which hastwo separate paths. This architecture increases the number of possible enhance-ment procedures (i.e., the number of paths from input to output) exponentiallyas the network depth grows, and consequently allows to address various types ofimage degradation with a single network

% \tyson{What are special in our model}
In general, URIE resembles U-Net~\cite{unet} to keep small size of intermediate features to be computationally efficient.
However, for each contracting and expanding stage, we've come up with a series of split-and-merge structure in which two separate branches are executed in parallel and merged using selective attention, letting URIE have variety of choices to process images depending on latent degradation type.
By utilizing aforementioned advantages, URIE allows the entire network to be computationally efficient without having to be too deep, and can handle various and latent degradations.
The remainder of this section describes thorough details of URIE with its design points.

% To deal with various corruptions, our network splits for each stage to ensure multiple feed-forward paths. Each stage takes feature from previous one, feeding them to two different convolution layers with instance and batch normalization layer.
% Resulting features are integrated with selective attentions through squeeze-excitation block. 

\subsection{Model architecture}

% ======================================================================
% FIGURE START
\begin{figure*} [!t]
\centering
% \includegraphics[width = 1 \textwidth]{figures/fig_arch.pdf}
\includegraphics[width = 1 \textwidth]{figures/fig_selective_path.pdf}
% \includegraphics[width = 1 \textwidth]{figures/fig_selective_path.pdf}
% \fbox{\rule{0pt}{2in} \rule{1\linewidth}{0pt}}
\caption{
Details of the selective enhancement module of URIE.
} 
\vspace{-2mm}
\label{fig:selective_path}
\end{figure*}
% FIGURE END
% ======================================================================


As mentioned, URIE adopts U-Net~\cite{unet} like structure, which consists of contracting and expanding path. 
% Each intermediate feature in the contracting path are concatenated to the corresponding feature of the expansive path.
Having such structure, URIE could achieve better computational efficiency compared to classical image enhancement models thanks to shrinking spatial sizes of intermediate features.
In more details, however, URIE has its own way of processing each contracting and expanding stage different from that of U-Net.
For each stage, we conduct Batch Normalization (BN)~\cite{Batchnorm} and Instance Normalization (IN)~\cite{Instancenorm} and feed them to different convolution layers.
Then we integrate resulting features using selective attention and feed them to next stage.
By using such scheme, URIE can have exponential feed-forward paths to cope with multiple latent degradation factors, keeping its computational advantages.
URIE also has skip connection between input and output to maintain performance on images without corruption, which is often the case in the real world.
% By using such scheme, URIE can deal with individual operation depending on the latent degradation and increases versatile enhancement ability in the face of not a just single degradation type but several types.
% By gradually shrinking the spatial size of intermediate features in the contracting path, URIE can reduce its computational overhead which has been a bottleneck in classical image enhancement models.
% Also, it has a residual path to connect from beginnings to end to only generate residual image in an enhancement part.
% In addition, this split-and-merge structure ensures a number of possible enhancement procedures (i.e., the number of paths from input to output) exponentially as depth grows since paths gets doubled for each stage the image passes. It can allows our network to be light-weight and speedy without having to be too deep.

From now on, we examine our proposed two-split branch with different normalization in each stage(block or module) to tackle multiple degradation problem. 
Let $\mathrm{X} \in \mathbb{R}^{H \times W \times C}$ be the input of stage. 
Two outputs $\mathrm{U, V} \in \mathbb{R} ^ {H \times W \times C'}$ are processed by following separate normalization and convolution operation in each branch as:
\begin{align}
    U = {K}_{1} * \sigma(BN(X)), \\
    V = {K}_{2} * \sigma(IN(X))
\end{align}
where * is the convolution operation and, $\sigma$ and ${K}_{i} \in \mathbb{R}^{k \times k \times C \times C'}$ denote an activation function and convolution kernel weight of branch ${i}$. 
To integrate two output features, we calculate selective attention for each branch from the fused output~$F$ via element-wise summation:
\begin{align}
    F = U + V
\label{fuse}
\end{align}

A sequence of patch-wise average pooling and two Fully Connected (FC) layers is applied to the fused output.
Let $z \in \mathbb{R}^{h \times w \times C'}$ denotes the pooled feature and average pooling operation is applied to embed the fused ouptut over the size ($\frac{H}{h}, \frac{W}{w}$) in each patch:
\begin{align}
    {z}_{i,j,c} = \cfrac{1}{m \times n} \sum_{x=m*i+1}^{m*(i+1)}\sum_{y=n*j+1}^{n*(j+1)}{F}_{x,y,c}
\end{align}
where $m = \frac{H}{h}, n = \frac{W}{w}$.
After that, embedding feature is flattened to the 1-dimension vector and two FC layers are applied to generate two attention maps, $\textbf{a}$ and $\textbf{b}$. 
\begin{align}
    s = {W}_{\alpha}({T}_{flat}(z))\\
    \textbf{a} = {W}_{\beta_1}(\delta(s)), \textbf{b} = {W}_{\beta_2}(\delta(s))
\label{attention}
\end{align}
where ${W}_{\alpha} \in \mathbb{R}^{\frac{(h \cdot w \cdot C')}{r} \times (h \cdot w \cdot C')}$, ${W}_{\beta_1}, {W}_{\beta_2} \in \mathbb{R}^{(h \cdot w \cdot C') \times \frac{(h \cdot w \cdot C')}{r}}$, $r$ is reduction ratio as used in~\cite{hu2018squeeze,Li2019_SKNet} to form a bottleneck between two FCs, and $\delta$ is LReLU activation. \juwon{why fcs are applied, reshape operation from a to a'?}
Softmax operator is applied between each element of $\textbf{a}$ and $\textbf{b}$ to obtain final attention map $\textbf{a}', \textbf{b}' \in \mathbb{R}^{h \times w \times C'}$:
\begin{align}
    {\textbf{a}'}_{i,j,c} = \cfrac{\exp{({a}_{i,j,c}})}{\exp{({a}_{i,j,c})} + \exp{({b}_{i,j,c}})}, {\textbf{b}'}_{i,j,c} = \cfrac{\exp{({b}_{i,j,c})}}{\exp{({a}_{i,j,c})} + \exp{({b}_{i,j,c})}}
\label{softmax_att}
\end{align}
The attentions are meant to help selective usage over two differently processed features depending on the latent degradation type to produce the final output $Y \in \mathbb{R}^{H \times W \times C'}$:
\begin{align}
    Y = {f}_{interp}(\textbf{a}') \cdot U + {f}_{interp}(\textbf{b}') \cdot V
\label{output}
\end{align}
where ${f}_{interp}$ is an interpolation function to match the spatial size.
\juwon{pooling, unpooling operation is omitted}
\juwon{Figure}

To capture different characteristic of image, different normalization methods are applied, BN and IN. 
Batch normalization are traditionally essential element for training CNN, but instance normalization was proposed for style normalization and has been widely adopted in style transfer~\cite{Instancenorm}. 
Since there are several degradation types, like fog and frost, which generally change image style, we use IN for one branch to manipulate degradation-specific style information. 
Weighted attention between two outputs which was processed by separate normalization and convolution help to handle variety of degradation type and level.
\juwon{closing remarks}

% \juwon{Aspect of Light-weigh, Handing various and latent factors of degradation}


% \tyson{Explain reason why we adopt scheme from SKNet - to consider multi-degradations, different normalization scheme} 
% + An image can be represented with its mean and standard deviation, often considered as image's style.
% + However, with corruptions\tyson{or degradations?} introduced from \cite{Hendrycks2019_ImageNetC}, we confirmed that images \emph{style} changes dramatically.
% \tyson{insert figure that shows statistical difference before and after corruption is applied}
% The original intuition of SKNet is to take advantage of using convolved features from different kernel sizes.
% + To keep compact size of the network and To have many forward paths to consider various degradations, we adopt selective kernel scheme from selective kernel network\recap{(cite)}.
% + This way we can ensure multiple forward paths even if we don't make our networks too deep, since paths gets doubled for each stage the image passes.
% + Different thing from SKNet, our network has IN and BN for each branch and we don't utilize different kernel sizes.
% \tyson{explain why we made our model to have IN and BN + SKnet?}
% + Different from SKNet architecture, we put BatchNorm layer and Instance Norm layer with ReLU activation layer in front of the convolution layer.
% + Our reformed version of model includes two separate paths for each stage, including its own normalization and convolution layers as shown in Fig. 2.

\subsection{Training Scheme}
In this section, we describe how we train URIE.
We suggest novel training scheme, which is to train via coupled recognition network to learn enhancing semantic features of images.
In order to do that, we use task-specific loss from pretrained network for URIE to learn improve more important characteristics with limited resources.
Specifically, we adopt classification task as our training task and recognition model as ResNet-50~\cite{resnet}
During training, we couple URIE with fixed pretrained ResNet50~\cite{resnet} and train whole model with classification signal.
In this way, with mainitaining computational efficiency, URIE can concentrate its enhancement on salient objects in the image as opposed to classical restoration models.
For dataset, we use ImageNet-C~\cite{Hendrycks2019_ImageNetC}, which is corrupted version of ImageNet~\cite{Imagenet}, for semantic image enhancement.
We use 16 corruptions as seen corruptions including clean version of the image in addition to 15 training corruptions amoing 19 suggested in~\cite{Hendrycks2019_ImageNetC}.
Remaining 4 corruptions are used for testing our model for its generalization ability.
For ImageNet-C~\cite{Hendrycks2019_ImageNetC} training, we resize input images to (256, 256) and random crop to (224, 224) with random horizontal flip for data augmentation.
% We address in this way URIE can learn how to fully with huge amount of training dataset and numerous combinations of corruption and severity.

% For universal image enhancement, we use ImageNet~\cite{Imagenet} dataset with 15 corruptions among 19 introduced in \cite{Hendrycks2019_ImageNetC} so that our network can learn variety of enhancement techniques depending on latent degradations.
% Additionally, we add clean type to 15 corruptions during runtime to let URIE learn how to deal with already-fine images, which is necessary in the real world.
% % We generate images with random corruption and severity during the training so that our network can learn numerous combinations of images, corruptions and severities.
% Among several recognition tasks, we chose classification with ResNet-50~\cite{resnet} as our training task since it is the most basic and general task to learn how to enhance necessary details of the image.
% We chose ResNet50 ~\cite{resnet} for its moderate complexity and verified performances on image recognition.
% Since we assume learning restoration is not an optimal solution for image recognition, we use task-specific loss via coupled recognition network.
% By doing so, URIE can learn how to enhance image depending on latent degradation type and add necessary details to input images in terms of recognition.
% - Similar to many other image restoration works(cite denoising, dehazing...), our network is designed to generate residual image.
% - We train our model with classification loss only\tyson{or classification + reconstruction loss} while recognition model remains fixed during the training.
% - The training dataset we used for our task is ILSVRC2012 and CUB-200-2011. 
% - Our overall training strategy is very simple: simple classification task.
% - All you need to do is to let images pass our model before it goes into recognition model. 
% - We used Adam optimizer to train our network and used 227 x 227 image size.
% - The batch size is fixed to 32, and we used learning rate decay at a period of 10 epochs.
% - The initial learning rate is 1e-3.
% - Our training ends after 100 epochs. 

\subsection{Discussion} 
Traditional restoration work has redundant but inevitable need for recovering unnecessary details of the image, which requires heavy computational resources.
Different from classical image enhancement problem, URIE tries finding salient object from input and properly enhance with residual image it generates, regardless of how much the output image becomes similar with ground truth image.
Although images URIE generates may be distant from ground truth image in pixel intensity, feeding image with adjusted salient regions to following recognizer turns out to be very helpful rather than feeding restored image. 
In Figure~\ref{fig:cub_example}, sequence of images are shown to verify URIE is working on salient region of the images.
Examining URIE's output, which is column (b), it seems image is de-snowed in general.
However, in detail, pixels in region of birds are more carefully enhanced compared to background pixels.
Gradient CAM is also changed to be similar with that of clean image after applying URIE on distorted images, which justifies that URIE works for image recognition.
Moreover, in computational efficiency, URIE shows remarkable improvement in computational need adopting U-Net~\cite{unet} like architecture as shown Table \ref{tab:model_complexity_comparison}.
URIE requires 7 times less computation compared to current sota model~\cite{OWAN_CVPR19}, which is critical considering its appliance to the field where requires speedy evaluation. 
% Learning from the task-specific loss via recognizer enables URIE to add\juwon{enhance} important features helpful for any recognition tasks. \juwon{shallow and(speedy?) using split-and-merge}
% Although image restoration task has the burden to recover unnecessary detail regardless of recognition, our network doesn't aim to recover overall image and care about irrelevant background or feature (qualitative result). 

Though our attention scheme is inspired by SKNet~\cite{Li2019_SKNet}, the proposed attention mechanism is specialized for utilizing differently normalized and processed features in selective way. \juwon{same kernel size in our branch, but minor difference}
Applying two different normalization followed by separate convolution grants versatile flexibility to our network as well as attention mechanism.
Moreover, using spatial and channel wise attention gives even greater range of choices rather than using channel attention only, which makes URIE more flexible to latent degradation type.
% To deal with several degradation types for enhancement, the combination of selective attention (or splite-and-merge?) structure and different normalization methods are clearly effective. \juwon{repeated..?}
% But, SKNet gets benefit from the use of multiple kernels and the adaptive selection mechanism among them. 


% ======================================================================
% FIGURE START
\begin{figure*} [!t]
\centering
% \includegraphics[width = 1 \textwidth]{figures/fig_arch.pdf}
\scalebox{0.4}{
\includegraphics[width = 1 \textwidth]{figures/fig_cub_discussion.pdf}
}
% \includegraphics[width = 1 \textwidth]{figures/fig_selective_path.pdf}
% \fbox{\rule{0pt}{2in} \rule{1\linewidth}{0pt}}
\caption{Example outputs of URIE, first row of (a) denotes input image with corruptions, (b) denotes output of URIE, and (c) is clean version of the image. Images in second row are corresponding gradient cam plotted with ResNet-50~\cite{resnet} pretrained on clean CUB
} 
\vspace{-2mm}
\label{fig:cub_example}
\end{figure*}
% FIGURE END
% ======================================================================

% There exists a few papers considering image restoration considering multiple unknown degradations, RL-Restore~\cite{RL-Restore_CVPR18} and OWAN~\cite{OWAN_CVPR19}
% However, they solve image restoration problem regardless of recognition task, which is a key difference with ours. 
% \juwon{Need to contain detail of RL-Restore?}
% Similar with our network, OWAN utilizes attention mechanism among multiple operation layers depending on the input. 
% However, URIE is more efficient than OWAN and covers more variety of degradation types to reflect real-world problem. 
% Interestingly, OWAN shows the improved performance on the high-level vision task (object detection), so we compared their result and ours with computational overhead in experiment section. 

% In more details, instance normalization de-style(?) images to make network focus more essential part of the image, while batch normalization branch constrain features not to 
% Corruptions seriously harm recognition quality erasing\tyson{disturb} critical\tyson{decisive, necessary} details of the image. 
% Classical image restoration works tried solving this with recovering missing parts of the image.
% However, restoring redundant\tyson{trivial} details\tyson{characteristics} has been causing unnecessary burden\tyson{workload} to the network.
% We therefore train our network with recognition loss\tyson{or recog + recon, rather than recon only}



==> _4_experiments_backup_20200305.tex <==
% !TEX root = TY_ECCV20.tex
\section{Experiments}
\label{sec:experiment}

% %% ======================================================================
% %% TABLE START
% \begin{table}[!t] \small
% \caption{Model complexity comparison in terms of the number of multiply-accumulate operations (MACs) (G), the number of parameters and net forward time.
% }
% \centering
% \begin{tabular}
% {@{}C{2cm}|@{}C{2cm}|@{}C{2cm}|@{}C{2cm}|@{}C{2cm}
% }
% \cline{1-5}
% Model     & DnCNN & RL-Restore & OWAN  & \multicolumn{1}{c}{URIE} \\ \hline
% MACs(G)   & 2.216 & 0.474      & 1.431 & 0.246                     \\
% PARAMS(M) & 0.558 & 0.196      & 0.391 & 0.672        \            \\ \hline
% \end{tabular}
% \vspace{0.1cm}

% \label{tab:model_complexity_comparison}
% \vspace{-2mm}
% \end{table}
% %% TABLE END
% %% ======================================================================

This section demonstrates the effectiveness of our method in various settings.
We verify that URIE is applicable to image classification, semantic segmentation and object detection with no retraining throughout numerous experiments.
In specific, the transferability of URIE is shown through its transfer test to unseen recognizers, datasets and tasks. 
Furthermore, we also show that URIE is applicable to real world datasets achieving the best performance compared to the current state-of-the-art models. 
\suha{don't understand clearly, have to revise; btw, transferability vs. universality?}

%% ======================================================================
%% TABLE START
% \begin{wraptable}{r}{5cm}
% \vspace{-1cm}
% \caption{Architecture detail}
% \vspace{0.4cm}
% \centering
% \scalebox{0.63}{
% \begin{tabular}{@{}C{0.5cm}|@{}C{2cm}|@{}C{4.5cm}@{}}
% \hline
% idx & Output & URIE \\ \hline  
% 1 & $N x N$ & $9 x 9, pad=4, 32$
% \\  \hline
% 2 & $N/2 x N/2$ &  
% \left[\begin{array}{c} 2 \times 2~\textrm{maxpool} \\  3 \times 3~\textrm{sconv},~64 \end{array}\right]   
% \\ \hline 
% 3 & $N/4 x N/4$ & $
% \begin{bmatrix}
% 2 \times 2,~\textrm{maxpool}
% \\ 
% 3 \times 3~\textrm{sconv},~64
% \end{bmatrix}$
% \\ \hline
% 4 &
% $N/2 x N/2$ &  
% $
% \begin{bmatrix}
% 2 \times 2,~\textrm{upsample}
% \\ 
% ~\textrm{concat(2, upsample(3))}
% \\
% 3 \times 3~\textrm{sconv},~32
% \end{bmatrix}
% $              
% \\ \hline
% 5&
% $N x N$ & 
% $
% \begin{bmatrix}
% 2 \times 2,~\textrm{upsample}
% \\ 
% ~\textrm{concat(1, upsample(4))}
% \\
% 3 \times 3~\textrm{sconv},~16
% \end{bmatrix}
% $
% \\ \hline
% 6 & $N x N$ & $3 x 3, 3$
% \\ \hline
% \end{tabular}
% \vspace{-1cm}
% }
% \label{tab:archi_detail}
% \end{wraptable}
%% TABLE END
%% ======================================================================
\subsection{Training Configuration}
Each training image is first resized to 256$\times$256, and cropped to 224$\times$224 and flipped horizontally at random for data augmentation.
Then it is degraded on-the-fly by the synthetic distortion generator of the ImageNet-C~\cite{Hendrycks2019_ImageNetC}, where the type and intensity of distortion are determined at random.
Note that only 15 distortion classes among 19 are used during training as described in Sec.~\ref{sec:training_urie}.
% the type of distortion is randomly sampled from the 15 classes enumerated in Sec.~\ref{sec:training_urie} while its intensity is determined among 5 levels at random.
For optimizing the model, we employ Adam~\cite{Adamsolver} with learning rate 0.001, and decay the learning rate every 8 epochs by 10.
Our model is trained for 30 epochs with minibatches of size 112.

\iffalse
% - very details of our model
%   -- the number of layers
%   -- the number of parameters 
%   -- FLOPs
%   >> may be different for different versions of our model
%   >> would be nice to summarize the above numbers in a table and to compare them with those of other enhancement networks, RL-Restore and OWAN, to show the computational efficiency of our model (is it really "light-weight"?)
In this section, we explain training configurations and implementation details of URIE.
Our architecture consists of two normal convolutions and four contracting and expanding phases as shown in Table \ref{tab:archi_detail}.
The very first convolution adopts $9\times9$ kernel with padding size 4 to grab sufficient information from an input image.
The other convolution layers use $3\times3$ kernels with padding size 1.
% Every contracting stages reduces input spatial size by 2 first, then feed resulting feature to selective convolution block.
% In the block, we perform BN and IN separately followed by LReLU activation layer. 
% Resulting features are then fed to convolution layers with kernel size of 3 (which is the same in all selective blocks), keeping its spatial size. 
% Afterwards, average pooling is applied reducing spatial size of the feature to 4 x 4.
% Then we flatten the whole features and generate spatial- and channel- wise\tyson{FIX:wording} attention through squeeze and excitation manner with reduction ratio 16 and using 2 fully connected layers with ReLU activation function.
% The attentions are adjusted using element-wise softmax to maintain multiplied features' scale as the same.
% For the last stage, we apply final convolution layer with kernel size of 3 reducing channel size to 3, which is the same as input.
In training, we employ the Adam optimizer~\cite{Adamsolver} with learning rate 0.001 and decay the learning rate by 10 every eight epochs.
We trained our model for 30 epochs with batch size 112.
\fi


% To learn universally applicable image enhancement manner, we train URIE on ImageNet~\cite{Imagenet} with generated on-the-fly random corruption and severity proposed in~\cite{Hendrycks2019_ImageNetC}.
% We use 15 corruptions among total 19 corruptions to use remaining corruptions for testing, which is the same setting as~\cite{Hendrycks2019_ImageNetC}.
% In training, a corruption is randomly selected from 16 training splits(15 + original image) then applied to input image with random severity.
% For validation, we generate csv file containing validation image, corruption pair so that we can reproduce the same results with the same model. 

% - about training 
%   -- dataset
%       --- ImageNet-C
%       --- corruption types and our seen/unseen split
%       --- setting for corruption levels during training
%       --- etc.
%   -- recognizer: resnet-xx
%   -- hyper-parameter setting
% - baselines
%   -- RL-Restore (CVPR'18) and OWAN (CVPR'19)
%   -- using the original models provided by authors, and those trained in the same setting as ours

\subsection{Experimental Configurations}
We here describe our experimental settings including datasets and models.
For evaluation of our model, we use the test sets of widely used image recognition datasets including ImageNet~\cite{Imagenet}, VOC~\cite{Pascalvoc}, and CUB~\cite{CUB200}.
For each dataset, we generated three versions of its test set.
(1)~\emph{Clean:}
original uncorrupted images,
(2)~\emph{Seen}: 
images with corruptions randomly sampled from the set of seen corruptions, and
(3)~\emph{Unseen}:
images with corruptions randomly sampled from the set of unseen corruptions.
We did not generate the datasets on-the-fly but prior to evaluation so that they are fixed during evaluation.

To verify the effectiveness of URIE, we evaluate the recognition performance of different combinations of recognizers and image enhancement modules: Baseline, OWAN+, URIE(MSE)+, and URIE+.
The recognizers are trained on the original clean images of each target dataset.
% Baseline is the baseline approach that uses recognizers with no enhancement modules.
OWAN+ indicates a combination of a recognizer with OWAN~\cite{OWAN_CVPR19}, which is the state-of-the-art image restoration method that is designed to deal with images with multiple unknown types of corruption.
We trained OWAN using an L1 loss as proposed in \cite{OWAN_CVPR19} with our training dataset.
URIE(MSE)+ indicates a combination of a recognizer with URIE(MSE), an image restoration-oriented variant of URIE, which is trained using a mean-squared-error (MSE) loss.
Finally, URIE+ indicates a combination of a recognizer with our proposed model, URIE.
OWAN+ and URIE(MSE)+ are included to investigate the effectiveness of URIE over classical restoration approaches.

% This section describes our experimental settings with related to dataset and models used for evaluation.
% For each target dataset used in experiments, we generated 3 versions for evaluation.
% (1)~\emph{Clean}: 
% Original test images from official dataset without any corruptions. 
% % Performance over clean dataset still matters as well as on corrupted dataset, since images are not always corrupted in the wild\tyson{real world}.
% (2)~\emph{Seen and Unseen}: 
% Test images with corruptions randomly selected from seen and unseen corruptions. We split seen and unseen split as proposed in~\cite{Hendrycks2019_ImageNetC}. For each dataset, we generate fixed validation list consists of combination of test image, corruption and severity for parallel comparison between models.
% We suppose there already exists a recognizer pretrained on clean data of target dataset, we evaluate performances of target task with and without URIE in the presence of corruptions.
% Regarding all our experiments, note that \textbf{we never finetune} URIE on any other tasks nor dataset except aforementioned training procedure on ImageNet-C~\cite{Hendrycks2019_ImageNetC}.

% To address URIE has better enhancement ability over classic restoration-specific trained model, we compare following 3 models.
% (1)~\emph{OWAN}~\cite{OWAN_CVPR19}: We trained model introduced in OWAN~\cite{OWAN_CVPR19} following the exact same scheme introduced in the paper with our dataset. 
% (2)~\emph{URIE(MSE)}: URIE trained with mean squared error(MSE) between input and ground truth images to verify restoration is rather ineffective for image recognition. We denote this model as MSE in experiment section to avoid any confusion between URIE trained with task-specific loss.
% (3)~\emph{URIE}: The model we suggest in this paper, trained with task-specific loss as described training scheme section.  
% Note that all the baseline results are measured with \textbf{recognizers pretrained on clean dataset only.}

%% ======================================================================
%% TABLE START
\begin{table}[!t] \small
\centering

\caption{Quantitative Evaluation on ImageNet-C, numbers in parenthesis show relative performance compared to baseline.

}
\scalebox{0.7}{
\begin{tabular}{@{}C{1cm}|@{}C{1.8cm}@{}C{1.8cm}@{}C{1.8cm}|@{}C{1.8cm}@{}C{1.8cm}@{}C{1.8cm}|@{}C{1.8cm}@{}C{1.8cm}@{}C{1.8cm}@{}}
\multirow{2}{*}{}   & \multicolumn{3}{c|}{OWAN+}  & \multicolumn{3}{c|}{URIE(MSE)+} & \multicolumn{3}{c}{URIE+}  \\ \cline{2-10} & \multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Seen} & \multicolumn{1}{c|}{Unseen} & \multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Seen} & \multicolumn{1}{c|}{Unseen} & \multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Seen} & \multicolumn{1}{c}{Unseen} \\ \hline
V16 & 69.8 \red{(-0.2)} & 31.6 \green{(+2.0)} & 39.8 \green{(+0.8)} & 59.5 \red{(-10.5)} & 32.3 \green{(+2.7)} & 38.1 \red{(-0.9)} & 67.1 \red{(-2.9)} & 42.4 \green{(+12.8)} & 44.8 \green{(+5.8)} \\
R50 & 74.4 \red{(-0.4)} &  42.6 \green{(+2.0)} & 50.3 \green{(+1.2)} & 66.7 \red{(-7.8)} & 44.5 \green{(+3.9)} & 49.3 \green{(+0.2)} & 72.9 \red{(-1.6)} & 55.1 \green{(+14.5)} & 56.5 \green{(+7.4)}  \\
R101& 75.9 ( 0.0) & 47.4 \green{(+1.5)} & 54.6 \green{(+0.8)} &  68.8 \red{(-7.1)} & 50.0 \green{(+4.1)} & 54.0 \green{(+0.2)} & 74.1 \red{(-1.8)} & 57.8 \green{(+11.9)} & 59.4 \green{(+5.6)} 
\end{tabular}
}
\label{tab:classification_on_imagenet}
\end{table}
%% TABLE END
%% ======================================================================

%% ======================================================================
%% TABLE START
\begin{table}[!t] \small
\centering
\caption{Quantitative Evaluation on CUB-C, numbers in parenthesis show relative performance compared to baseline.
}
\scalebox{0.7}{
\begin{tabular}{@{}C{1cm}|@{}C{1.8cm}@{}C{1.8cm}@{}C{1.8cm}|@{}C{1.8cm}@{}C{1.8cm}@{}C{1.8cm}|@{}C{1.8cm}@{}C{1.8cm}@{}C{1.8cm}@{}}
\multirow{2}{*}{}   & \multicolumn{3}{c|}{OWAN+}  & \multicolumn{3}{c|}{URIE(MSE)+} & \multicolumn{3}{c}{URIE+}  \\ \cline{2-10} & \multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Seen} & \multicolumn{1}{c|}{Unseen} & \multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Seen} & \multicolumn{1}{c|}{Unseen} & \multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Seen} & \multicolumn{1}{c}{Unseen} \\ \hline
V16 & 79.1 ( 0.0) & 50.4 \green{(+4.2)} & 42.3 \green{(+1.7)} & 68.5 \red{(-11.6)} & 50.5 \green{(+4.3)} & 39.6 \red{(-1.0)} & 77.9 \red{(-1.2)} & 58.8 \green{(+12.6)} & 48.9 \green{(+8.3)} \\
R50 & 84.6 ( 0.0) & 52.8 \green{(+3.3)} & 48.2 \green{(+1.2)} & 76.5 \red{(- 8.1)} & 58.4 \green{(+8.9)} & 49.3 \green{(+2.1)} & 83.7 \red{(-0.9)} & 64.7 \green{(+15.2)} & 54.9 \green{(+7.7)}  \\
R101& 84.9 \red{(-0.1)} & 55.5 \green{(+3.6)} & 48.5 \green{(+1.8)} & 76.2 \red{(- 8.8)} & 59.9 \green{(+8.0)} & 50.5 \green{(+3.8)} & 84.1 \red{(-0.9)} & 67.1 \green{(+15.2)} & 56.6 \green{(+9.9)}
\end{tabular}
}
\label{tab:classificaion_on_cub}
\end{table}
%% TABLE END
%% ======================================================================

% ======================================================================
% FIGURE START
\begin{figure*} [!t]
\centering
% \includegraphics[width = 1 \textwidth]{figures/fig1.pdf}
\includegraphics[width = 1 \textwidth]{figures/fig_cub_qual.pdf}
\caption{
Qualitative examples on CUB-C classification. In each grid, first column is input image and each following columns show output image of OWAN, URIE(MSE), URIE and ground truth. Every even-numbered row shows corresponding gradCAM of image right above measured from pretrained 3rd basic block of ResNet-50~\cite{resnet}}
\vspace{-1mm}
\label{fig:motiv}
\end{figure*}
% FIGURE END
% ======================================================================


\subsection{Performance Evaluation}
% - our goals
%   -- ablation study
%   -- demonstrating that our model is universally applicable to different architectures of the same task
We first compare the performance of URIE against the other models on classification on ImageNet-C.
In this comparison, we use a ResNet-50 classifier network trained on clean images of ImageNet~\cite{imagenet} as a recognizer, which is the model used to train URIE (Section \ref{sec:training_scheme}).
The first row (R50) in Table \ref{tab:classification_on_imagenet} shows the comparison result.
In the table, numbers in parantheses indicate relative performance gains compared to the baseline model.
The table shows that URIE(MSE) performs comparably against OWAN both for seen and unseen corruptions even though URIE(MSE) is about six times lighter in terms of computational load as shown in Table \ref{tab:model_complexity_comparison}.
The table also shows that URIE significantly outperforms all the other models both for seen and unseen corruptions, while shows performance close to that of the baseline, which is the upper bound.
This shows the effectiveness of our selective attention mechanism with task-specific training in dealing with multiple latent degradation types.

\paragraph{Transferability to other classifiers.}
To show the transferability of URIE, which is trained with a ResNet-50 classifier, we conduct another experiment,
where we use two different classifiers based on different network architectures: VGG-16, and ResNet-101 trained on clean images of ImageNet.
Regarding OWAN and URIE(MSE), we also use the same models as those in the previous experiment, as they are trained independently to recognisers.
%In the same way to the previous experiment, we measure the classification accuracy of each combination.
The second and third rows in Table \ref{tab:classification_on_imagenet} show the comparison of different models with VGG-16 and ResNet-101.
The results show that URIE still significantly outperforms all the other methods achieving performance gains similar to those for the ResNet-50 classifier in the first row,
which proves the transferability of URIE.

% The table shows that URIE significantly improves recognition accuracy both for seen and unseen corruptions compared to both OWAN and URIE(MSE), while 
% Moreover, URIE(MSE) 
% We compare URIE with OWAN and URIE only trained from reconstruction loss (MSE).
% Table \ref{tab:classificaion_on_imagenet} shows significant improvement of URIE on both Seen and Unseen validation. 
% Although OWAN has marginal superiority over URIEs on clean datset, URIE shows dominating performance compared to the other competitors on corruption set. URIE is very efficent than OWAN in the aspect of the number of computation (1.431 vs 0.246 in Table 1).
% It indicates our selective attention mechanism with task-specific training grants more capability dealing with multiple latent degradation types.
% In addition, to show the transferability of each model, we use identical enhancement model which was trained from Resnet50 (except URIE(MSE)) per each column in Table \ref{tab:classificaion_on_imagenet}.
% For different recognizers, we choose VGG16~\cite{vggnet} to show it is transferable to entirely different architecture, and ResNet101~\cite{resnet} to show it is even capable of transferring to the same kinds of network but more depth. URIE shows similar performance improvement on different architecture (first and third rows). 
% Comparison to URIE(MSE) shows that task-specific loss gives enhancement ability to concentrate on helpful feature for recognition. 

% We present quantitative results of 3 models on 3 versions of ImageNet~\cite{Imagenet} validation set in Table \ref{tab:classificaion_on_imagenet}.
% For clean dataset though, OWAN has marginal superiority over URIE and MSE version.
% However, for seen and unseen validation set, URIE dramatically increases classification accuracy.


% - target data
%   -- ImageNet validation images corrupted by seen/unseen factors
% As mentioned, we generate fixed validation set with seen and unseen corruption split for reproducibility. 
% Therefore, the following results are measured from same evaluation images with seen/unseen corruption splits. 
% - target model
%   -- ImageNet classifiers pretrained without considering corruptions
%   -- one used for training (resnet-xx)
% %   -- those not used for training (vgg-19, resnet-yy)


% First, we train our enhancement model with the ResNet50 pretrained on ImageNet.
% While training, we freeze recognition model so that our model could learn recognition friendly image enhancement.
% Then we evaluate our model with different recognition backbones such as vgg-16, resnet-50 and resnet-101 to show our model is agnostic to backbone recognizer in the same task.
% \textbf{Note that we never finetune our model in the evaluation phase.}

% - quantitative performance analysis 
%   -- ablation study
%       --- perf. of our model trained with different losses (recognition/reconstruction/both?)
%       --- perf. of our model trained with BN/IN/Both (if we have no time to do this on the ImageNet, consider CUB-C which is suboptimal though)
%   -- perf vs. corruption factors (seen/unseen)
%   -- perf vs. recognition nets
%   -- perf of other enhancement techniques (OWAN and/or RL-Restore) in terms of recognition performance and image quality
% - qualitative examples
%   -- comparisons between


%% ======================================================================
%% TABLE START
\begin{table}[!t] \small
\centering
\caption{Semantic segmentation performance of DeepLab.v3 on the VOC2012-C. The numbers in parenthesis indicate the differences from the baseline performance.
}
\scalebox{0.74}{
\begin{tabular}{@{}C{1.8cm}@{}C{1.8cm}@{}C{1.8cm}|@{}C{1.8cm}@{}C{1.8cm}@{}C{1.8cm}|@{}C{1.8cm}@{}C{1.8cm}@{}C{1.8cm}@{}}
\multicolumn{3}{c|}{OWAN+}  & \multicolumn{3}{c|}{URIE(MSE)+} & \multicolumn{3}{c}{URIE+}  \\
\hline
\multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Seen} & \multicolumn{1}{c|}{Unseen} & \multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Seen} & \multicolumn{1}{c|}{Unseen} & \multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Seen} & \multicolumn{1}{c}{Unseen} \\ 
\hline
78.7 \red{(-0.2)} &  58.2 \green{(+3.3)}   &  65.4\green{(+2.1)} & 78.1 \red{(-0.8)} & 60.1 \green{(+5.2)} & 63.6 \green{(+0.3)} & 78.6 \red{(-0.3)} & 67.0 \green{(+12.1)} & 67.2 \green{(+3.9)} \\
\end{tabular}
}
\label{tab:segmentation_on_voc}
\end{table}

% \begin{table}[!t] \small
% \centering
% \caption{Semantic Segmentation performance of DeepLab.v3 on the VOC2012-C. Numbers in parenthesis indicate the differences from the baseline performance.
% }
% \scalebox{0.69}{
% \begin{tabular}{@{}C{1cm}|@{}C{1.8cm}@{}C{1.8cm}@{}C{1.8cm}|@{}C{1.8cm}@{}C{1.8cm}@{}C{1.8cm}|@{}C{1.8cm}@{}C{1.8cm}@{}C{1.8cm}@{}}
% \multirow{2}{*}{}   & \multicolumn{3}{c|}{OWAN+}  & \multicolumn{3}{c|}{URIE(MSE)+} & \multicolumn{3}{c}{URIE+}  \\ \cline{2-10} & \multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Seen} & \multicolumn{1}{c|}{Unseen} & \multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Seen} & \multicolumn{1}{c|}{Unseen} & \multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Seen} & \multicolumn{1}{c}{Unseen} \\ \hline
% DL.v3 &  78.7 \red{(-0.2)} &  58.2 \green{(+3.3)}   &  65.4\green{(+2.1)} & 78.1 \red{(-0.8)} & 60.1 \green{(+5.2)} & 63.6 \green{(+0.3)} & 78.6 \red{(-0.3)} & 67.0 \green{(+12.1)} & 67.2 \green{(+3.9)} \\
% \end{tabular}
% }
% \label{tab:segmentation_on_voc}
% \end{table}
%% TABLE END
%% ======================================================================


% ======================================================================
% FIGURE START
\begin{figure*} [!t]
\centering
% \includegraphics[width = 1 \textwidth]{figures/fig1.pdf}
\includegraphics[width = 1 \textwidth]{figures/fig_seg.pdf}
\caption{
Qualitative examples on VOC2012-C segmentation. In each grid, first column is input image and each following columns show output image of OWAN, URIE(MSE), URIE and ground truth. Every even-numbered row shows corresponding segmentation prediction mask of image right above.
} 
\vspace{-2mm}
\label{fig:motiv}
\end{figure*}
% FIGURE END
% ======================================================================


%\subsection{Quantitative Evaluation on CUB-C}
% - our goals
%   -- ablation study (skip if we have no time)
%   -- demonstrating that our model is universally applicable to the same task with different data domain
\paragraph{Transferability to other data domains.}
To investigate the transferability of URIE to other image deomains, we conduct another experiment.
In this experiment, we apply URIE, which is trained on ImageNet-C, to the CUB-C dataset, which is a corrupted version of the Caltech-UCSD Birds 200-2011 (CUB) dataset~\cite{CUB200}.
The CUB dataset is a fine-grained dataset for classification, which is vulnerable to even minor changes.
We evaluate the performance of our model with different classifiers as done in Table \ref{tab:classification_on_imagenet}.
The classifiers are trained on the clean images in the CUB dataset.
The quantitative results in Table \ref{tab:classificaion_on_cub} show that URIE significantly outperforms all the other methods both for seen and unseen corruptions similarly to the results of the previous experiments.

% For different domain of data, we choose Caltech-UCSD Birds 200-2011 since fine-grained classification is vulnerable to even minor changes.
% We also evaluate our model with different architectures as used in 4.3.
% Quantitative results in Table \ref{tab:classificaion_on_cub} show URIE is more capable of enhancing images in the aspect of recognition, still minor loss in clean images compared to OWAN~\cite{OWAN_CVPR19}.
% Furthermore, URIE gives dramatic boosts to seen column, which indicates it is trained to enhance images from latent degradation type even with unknown domain of data.

% - target data
%   -- CUB validation images corrupted by seen/unseen factors
% - target model
%   -- CUB classifiers pretrained without considering corruptions
%   -- one used for training (resnet-xx)
%   -- those not used for training (vgg-19, resnet-yy)
%   >> choose only a single model if we do not have enough time to conduct all the experiments, resnet-18 is ok
% - quantitative performance analysis 
%   -- ablation study: perf. vs. our model's variants trained with different losses (recognition/reconstruction/both, skip if we have no time)
%   -- perf vs. corruption factors (seen/unseen)
%   -- perf vs. recognition nets (skip if we have no time)
%   -- perf of other enhancement techniques (OWAN and/or RL-Restore) in terms of recognition performance and image quality
% - qualitative examples
%   -- comparisons between our model and other enhancement techniques (OWAN): their output images, reconstruction performance, and recognition accuracy
%% ======================================================================
%% TABLE START
\begin{table}[!t] \small
\centering
\caption{Object detection performance of SSD300 on the VOC2007-C. The numbers in parenthesis indicate the differences from the baseline performance.
}
\scalebox{0.74}{
\begin{tabular}{@{}C{1.8cm}@{}C{1.8cm}@{}C{1.8cm}|@{}C{1.8cm}@{}C{1.8cm}@{}C{1.8cm}|@{}C{1.8cm}@{}C{1.8cm}@{}C{1.8cm}@{}}
\multicolumn{3}{c|}{OWAN+}  & \multicolumn{3}{c|}{URIE(MSE)+} & \multicolumn{3}{c}{URIE+} \\
\hline
\multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Seen} & \multicolumn{1}{c|}{Unseen} & \multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Seen} & \multicolumn{1}{c|}{Unseen} & \multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Seen} & \multicolumn{1}{c}{Unseen} \\ 
\hline
77.4 (0.0) &  51.3 \green{(+1.7)}   & 60.2 \green{(+0.9)} & 76.5 \red{(-0.9)} & 52.7 \green{(+3.1)} & 59.9 \green{(+0.6)} & 76.5 \red{(-0.9)} & 59.4 \green{(+9.8)} & 62.7 \green{(+3.4)} \\
\end{tabular}
}
\label{tab:detection_on_voc}
% \vspace{-2mm}
\end{table}
%% TABLE END
%% ======================================================================


% ======================================================================
% FIGURE START
\begin{figure*} [!t]
\centering
% \includegraphics[width = 1 \textwidth]{figures/fig1.pdf}
\includegraphics[width = 1 \textwidth]{figures/fig_detect.pdf}
\caption{
Qualitative examples on VOC2007-C detection. In each grid, first column is input image and each following columns show object detection result of OWAN, URIE(MSE), URIE and ground truth. 
} 
\vspace{-1mm}
\label{fig:motiv}
\end{figure*}
% FIGURE END
% ======================================================================

%\subsection{VOC-C Object Detection and Semantic Segmentaiton}
% - our goals
%   -- demonstrating that our model is universally applicable to the different recognition tasks
% - target data
%   -- VOC validation images corrupted by seen/unseen factors
% - target model
%   -- faster r-cnn pretrained on the VOC 2012 without considering corruptions
%   -- deeplab v2 pretrained on the VOC 2012 without considering corruptions
% - quantitative performance analysis 
%   -- perf vs. corruption factors (seen/unseen)
%   -- perf of other enhancement techniques (OWAN and/or RL-Restore) in terms of recognition performance and image quality
% - qualitative examples
%   -- comparisons between our model and other enhancement techniques (OWAN): their output images, reconstruction performance, and recognition accuracys
\paragraph{Transferability to other recognition tasks.}
In the next experiment, we examine the transferability of URIE to other recognition tasks beside classification.
In this experiment, we consider two recognition tasks: semantic segmentation and object detection.
Regarding semantic segmentation, we use DeepLab v3~\cite{chen2018encoder} with ResNet-101~\cite{resnet} as a segmentation network.
Regarding object detection, we use SSD~\cite{SSD} as an object detection network.
To evaluate the performance of URIE, we use corrupted versions of the Pascal 2007 and 2012 datasets~\cite{Pascalvoc}, which are referred to as VOC2007-C and VOC-2012-C, respectively.
Tables \ref{tab:segmentation_on_voc} and \ref{tab:segmentation_on_voc} compare the performance of different methods on semantic segmentation and object detection, respectively.
In both tasks, URIE performs superiorly to the other methods both for seen and unseen corruptions, while achieving slightly worse performance than the upper bound, which is the baseline performance,
even though URIE is trained with a different task on a different dataset.

% In this section, we prove URIE is also transferable to other recognition task besides classification.
% We choose Pascal VOC~\cite{Pascalvoc} 2007 and 2012 for semantic segmentation and object detection.
% We use DeepLab.v3~\cite{chen2018encoder} with ResNet-101~\cite{resnet} for segmentation and SSD~\cite{SSD} for object detection.
% Table \ref{tab:segmentation_on_voc} and Table \ref{tab:detection_on_voc} shows quantitative evaluation on aformentioned tasks over 3 models.
% URIE shows dominant performance compared to its competitors regardless of dataset split and task.
% It clearly shows that URIE is capable of adding general details of image which any recognition task can utilize.
% Moreover, by comparing to MSE version of URIE, results also indicate that typical restoration processes are hardly capable of enhancing images in the respect of recognition.

\paragraph{Real Degradation Image Dataset.}
We finally examine the performance of URIE on a dataset with real degradation to verify its usefulness in the real world.
In this experiment, we consider classification on two datasets: Haze-20 and HazeClear-20 proposed by Pei \etal~\cite{Pei_2018_ECCV}.
Haze-20 contains images of 20 categories with real-world haze, while HazeClear-20 contains haze-free images of the same 20 categories.
Note that real-world haze is more challenging for URIE as it is trained using only synthetic degradation.
Moreover, Pei \etal~showed that existing haze removal algorithms do not help improve the classification performance in their experiments.
Nevertheless, Table \ref{tab:classification_on_haze} shows that URIE is still able to improve the classification accuracy in the presence of real-world haze, while achieving performance close to the upper bound on HazeClear-20.


% For the last experiment, we test URIE on dataset with real haze~\cite{Pei_2018_ECCV} to verify its usefulness in the real world.
% We choose Haze-20~\cite{Pei_2018_ECCV} and HazeClear-20~\cite{Pei_2018_ECCV} which contains 20 categories of image with and without haze.
% Compared to previous dataset which are distorted by synthetic degradation, the dataset contains real world degradation. Moreover, although the real degradation was not considered while training URIE, URIE can enhance real haze image for recognition (fog is in ImageNet-C, but, synthetic).
% Table \ref{tab:classification_on_haze} shows quantitative results on proposed dataset.
% Considering Pei~\etal~\cite{Pei_2018_ECCV} addresses existing haze removal algorithms do not improve performances, result indicates URIE is also capable of dealing with real world degradation for recognition.
%% ======================================================================
%% TABLE START
\begin{table}[!t] \small
\centering
\caption{Evaluation on Real Degradation Image Dataset, numbers in parenthesis show relative performance compared to baseline.
}
\scalebox{1}{
\begin{tabular}{@{}C{1cm}|@{}C{1.8cm}@{}C{1.8cm}|@{}C{1.8cm}@{}C{1.8cm}|@{}C{1.8cm}@{}C{1.8cm}@{}}
\multirow{2}{*}{}   & \multicolumn{2}{c|}{OWAN+}  & \multicolumn{2}{c|}{URIE(MSE)+} & \multicolumn{2}{c}{URIE+}  \\ \cline{2-7} & \multicolumn{1}{c}{Haze} & \multicolumn{1}{c|}{HazeClear} & \multicolumn{1}{c}{Haze} & \multicolumn{1}{c|}{HazeClear} & \multicolumn{1}{c}{Haze} & \multicolumn{1}{c}{HazeClear} \\ \hline
R50 &  58.7 \green{(+1.7)} &  97.8 \red{(-0.1)} &  53.4 \red{(-3.6)} & 94.4 \red{(-3.5)} & 60.8 \green{(+3.8)} &  97.6 \red{(-0.3)} \\
\end{tabular}
}
\vspace{0.1cm}

\label{tab:classification_on_haze}
\vspace{-2mm}
\end{table}
%% TABLE END
%% ======================================================================

=============
% FIGURE START
\begin{figure*} [!t]
\centering
% \includegraphics[width = 1 \textwidth]{figures/fig1.pdf}
\includegraphics[width = 1 \textwidth]{figures/fig_haze.pdf}
\caption{
Qualitative examples on Haze-20. In each grid, first column is input image and each following columns show output image and gradient CAM result of OWAN, URIE(MSE), URIE. Each label denotes its top-1 prediction.
} 
\vspace{-2mm}
\label{fig:motiv}
\end{figure*}
% FIGURE END
% ======================================================================

